LEAD: Liberal Feature-based Distillation for Dense Retrieval

Knowledge distillation is often used to transfer knowledge from a strong teacher model to a relatively weak student model. Traditional methods include response-based methods and feature-based methods. Response-based methods are widely used but suffer from lower upper limits of performance due to their ignorance of intermediate signals, while feature-based methods have constraints on vocabularies, tokenizers and model architectures. In this paper, we propose a liberal feature-based distillation method (LEAD). LEAD aligns the distribution between the intermediate layers of teacher model and student model, which is effective, extendable, portable and has no requirements on vocabularies, tokenizers, or model architectures. Extensive experiments show the effectiveness of LEAD on widely-used benchmarks, including MS MARCO Passage Ranking, TREC 2019 DL Track, MS MARCO Document Ranking and TREC 2020 DL Track. Our code is available in https://github.com/microsoft/SimXNS/tree/main/LEAD.

==> tables/dataset_statistics.tex <==
\begin{table}[h]
\centering
% \small
% \resizebox{\columnwidth}{!}{
\caption{Statistics of the text retrieval datasets.} 
% \vspace{-1em}
\begin{tabular}{l|cccc}
\hline
\textbf{Dataset} & \textbf{Train} & \textbf{Dev} & \textbf{Test} & \textbf{\#Doc} \\
\hline
\textsc{MS-Pas} & 502,939 & 6,980 & - & 8,841,823 \\
\textsc{TREC-Pas-19} & - & - & 200 & 8,841,823 \\
\textsc{TREC-Pas-20} & - & - & 200 & 8,841,823 \\
\textsc{MS-Doc} & 367,013 & 5,193 & - & 3,213,835 \\
\textsc{TREC-Doc-19} & - & - & 200 & 3,213,835 \\
\textsc{TREC-Doc-20} & - & - & 200 & 3,213,835 \\
\hline
\end{tabular}
% }
% \vspace{-1em}
\label{tab:dataset}
\end{table}


==> tables/hyper.tex <==
\begin{table}[ht]
\centering
\caption{Hyper-parameters for distilling from 12-layer teachers to 6-layer DE. \textsc{Pas} denotes \textsc{MS-Pas}, \textsc{TREC-Pas-19} and \textsc{TREC-Pas-20}. \textsc{Doc} denotes \textsc{MS-Doc}, \textsc{TREC-Doc-19} and \textsc{TREC-Doc-20}. 12DE, 12CB, 12CE denote using 12-layer DE, 12-layer CB and 12-layer CE as the teacher model, respectively.}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|cc}
\hline
\textbf{Setting} & \textbf{Parameter} & \textbf{\textsc{Pas}} & \textbf{\textsc{Doc}} \\ \hline
\multirow{8}{*}{Global} & Max Query Length   & 32     & 32     \\
& Max Passage Length & 144    & 480    \\
& Training Step      & 5e4    & 5e4  \\
& Learning Rate      & 5e-5   & 5e-5   \\
& Warmup Proportion  & 0.1    & 0.1    \\ 
& Distillation Temperature    & 1      & 1      \\
& Distillation Layer Number   & 5     & 6     \\
& Layer Selection Temperature & 10     & 10     \\\hline
\multirow{2}{*}{12DE}  & Batch Size         & 80    & 48     \\
& Negative Size      & 16     & 16     \\\hline
\multirow{2}{*}{12CB}  & Batch Size         & 80    & 48     \\
& Negative Size      & 16     & 16     \\\hline
\multirow{2}{*}{12CE}  & Batch Size         & 16    & 8      \\
& Negative Size      & 15     & 15     \\\hline
\end{tabular}
% }

\label{tab:6-layer hyper}
\end{table}


\begin{table*}[ht]
\centering
\caption{Hyper-parameters for distilling from 24-layer teacher to 12-layer DE (24CB $\rightarrow$ 12DE).}

% \resizebox{\textwidth}{!}{
\begin{tabular}{l|cccccc}
\hline
\textbf{Parameter} & \textbf{\textsc{MS-Pas}} & \textbf{\textsc{TREC-Pas-19}} & \textbf{\textsc{TREC-Pas-20}} & \textbf{\textsc{MS-Doc}} & \textbf{\textsc{TREC-Doc-19}} & \textbf{\textsc{TREC-Doc-20}} \\ \hline
Max Query Length   & 32     & 32    & 32     & 32   & 32  & 32  \\
Max Passage Length & 144    & 144   & 144    & 480  & 480 & 480  \\
Batch Size         & 40     & 32    & 32     & 16   & 16  & 16  \\
Negative Size      & 16     & 16    & 16     & 8    & 8   & 8  \\
Training Step      & 5e4    & 5e4   & 5e4    & 5e4  & 5e4 & 5e4  \\
Learning Rate      & 2e-5   & 2e-5  & 2e-5   & 2e-5 & 2e-5& 2e-5  \\
Warmup Proportion  & 0.2    & 0.2   & 0.2    & 0.3  & 0.2 & 0.4  \\
Distillation Temperature    & 1   & 1   & 1  & 1    & 1  & 1  \\
Distillation Layer Number   & 11  & 11  & 10  & 11  & 9  & 11  \\
Layer Selection Temperature & 10  & 10  & 10  & 10  & 10 & 10  \\
\hline
\end{tabular}
% }
\label{tab:12-layer hyper}
\end{table*}
